Decoupling Skill Learning from Robotic Control for Generalizable Object Manipulation

Recent works in robotic manipulation through reinforcement learning (RL) or imitation learning (IL) have shown potential for tackling a range of tasks e.g., opening a drawer or a cupboard. However, these techniques generalize poorly to unseen objects. We conjecture that this is due to the high-dimensional action space for joint control. In this paper, we take an alternative approach and separate the task of learning 'what to do' from 'how to do it' i.e., whole-body control. We pose the RL problem as one of determining the skill dynamics for a disembodied virtual manipulator interacting with articulated objects. The whole-body robotic kinematic control is optimized to execute the high-dimensional joint motion to reach the goals in the workspace. It does so by solving a quadratic programming (QP) model with robotic singularity and kinematic constraints. Our experiments on manipulating complex articulated objects show that the proposed approach is more generalizable to unseen objects with large intra-class variations, outperforming previous approaches. The evaluation results indicate that our approach generates more compliant robotic motion and outperforms the pure RL and IL baselines in task success rates. Additional information and videos are available at https://kl-research.github.io/decoupskill

==> 2Relatedwork_old.tex <==
\section{RELATED WORK}

\begin{figure}
\centering
\includegraphics[width=1.03\linewidth]{figs/pipeline_new4.png}
\caption{\textbf{Architecture of the proposed system.} As shown in the yellow block, we use two simple PointNet\cite{qi_pointnet_2017} modules to separately perceive static (e.g. size of an object) and dynamic (e.g. current position of a handle) states. These are inputs to a SAC RL framework to learn how to control the disembodied end-effector, realizing a 6-DOF motion skill. Through knowledge of the robot's physical model, QP is used to effect optimization of the joint dynamics of the whole-body robot.}
\label{fig:pipeline}
\end{figure}

Robot learning for manipulation skills has been intensively studied in recent years. The dominant methods are reinforcement learning and imitation learning. 
An extensive survey of existing methods can be found in Kroemer's work \cite{kroemerreview}. 
However, robotic manipulation of complex objects through controlling high-DoF robots remains a challenging problem.

Recent works apply a variety of RL algorithms for robotic manipulation \cite{gu_deep_2017, kalashnikov_qt-opt_2018, yamada_motion_2020, liu_distilling_2021}.
% Gu et al. \cite{gu_deep_2017} deploy the classical off-policy deep Q-Learning network (DQN) for the door opening task. 
% % They deploy multiple real robots for parallel training and apply asynchronous policy updating. 
% Kalashnikov et al. \cite{kalashnikov_qt-opt_2018} exploit the DQN method to learn robust grasping strategies and non-prehensile pre-grasp manipulations. 
%Wu et al. \cite{wu_vat-mart_2021} present a policy-gradient SAC method for articulated object manipulation tasks. 
% To improve the pure RL policy, 
% Moreover, Yamada et al. \cite{yamada_motion_2020} propose a motion planner augmented soft actor-critic (SAC) algorithm for manipulation in obstructed scenes. In contrast, Liu et al.\cite{liu_distilling_2021} argue that the classical motion planner is not robust to state estimation error so they distill the planner into a visual control policy via behavior cloning. 
However, productive exploration has always been a challenge for robotic RL due to the complex dynamics of high-DOF robots. Many works have looked into decomposing the action space into higher-level policy and lower-level control to improve sampling efficiency and task performance. Exploiting predefined action primitives (e.g., lift, move, slide) is a convenient way to reduce the action space dimensions\cite{dalal_accelerating_2021, pertsch_accelerating_2020, xia2021relmogen}, but it requires manual specification of the robot behaviors.
% Dalal et al. \cite{dalal_accelerating_2021}  specify a library of robot action primitives and learn an RL policy to parameterize these primitives. Pertsch et al. \cite{pertsch_accelerating_2020} learn a  prior over skill primitives from offline agent experiences. Similarly, Xia et al. \cite{xia2021relmogen} learn a motion generator to execute designed subgoal motions of arm and base for navigation and mobile manipulation. 
% However, these methods require manual design of the primitive robot behaviors.
% Another line of research regarding choosing action space looks into 
Another approach regarding choosing action space is operational space control (OSC) \cite{khatib1987osc, peters2007reinforcement, wong2022oscar}, which requires a precise mass matrix to map the desired EE motions into joint torques. 
%Peters et al. \cite{peters2007reinforcement} and Wong et al. \cite{wong2021oscar} learn the mapping function 
%or inferring the relevant dynamics parameters from online trajectories 
% for robust motion control. 
Martin et al. \cite{martin-martin2019variable} compare OSC and other control modes in EE space and joint space using the Robosuite \cite{zhurobosuite} simulated environment and demonstrate that OSC usually outperforms other controllers in contact-rich tasks. However, in the presence of inaccuracies in dynamics modeling, OSC's performance quickly deteriorates \cite{nakanishi2008operational,wong2022oscar}. Our method shares a similar motivation with OSC-based RL, but our agent is a disembodied manipulator rather than a complete robot, without the need for high-fidelity modeling of the mass matrix during RL training.
Furthermore, this work presents category-level generalizability over various objects in the ManiSkill environment, while tasks in Robosuite typically focus on a single scene.

%These methods can also be viewed as a fixed-option hierarchical RL \cite{sutton2018reinforcement} where the options are their low-level control policies such as action primitives.

Imitation learning has usually been considered as a more sampling-efficient approach, but high-quality demonstrations that can be directly employed on robot motors are usually difficult to collect \cite{fang_survey_2019}. Shen et al. \cite{shen2022gail} propose a generative adversarial self-imitation learning method and a balancing expert buffer to mitigate the issues in ManiSkill's demonstration trajectories. IL with these techniques shows remarkable improvements in manipulation policy learning, but in this work, we focus more on learning from interactions.

% RL and IL are not strictly exclusive \cite{wang_goal-auxiliary_nodate, kulak_combining_2021}. In this work, we focus on learning an RL policy from scratch by our agent interacting with training instances.
% Wang et al. \cite{wang_goal-auxiliary_nodate} propose a goal-auxiliary policy-gradient RL algorithm using behavior cloning (BC) to initialize the policy model. Kulak et al. \cite{kulak_combining_2021} jointly learn from the demonstration trajectories and the online experiences of the robot by actively choosing between the two learning modalities. 

Another highly related topic is robotic vision for articulated object manipulation. Mo et al. \cite{mo_where2act_2021} and Wu et al. \cite{wu_vat-mart_2021} introduce  encoder-decoder networks to extract affordance maps and predict action proposals or trajectory proposals attached to the 3D representations of objects. Eisner et al. \cite{eisner2022flowbot3d} also implement a neural network to estimate point-wise motion directions called articulation flow for the point cloud observations. Similarly, Xu et al. \cite{xu2022umpnet} propose to estimate the motion directions and potential moving distances of the articulated parts using only a single image as input. In contrast, Mittal et al. \cite{mittal2022articulated} explicitly infer the articulation properties such as joint states and part-wise segmentation by giving object categories. These methods are object-centric representation learning and more focus on object articulation properties, usually leaving the next manipulation stage in a simplified way (e.g., a perfect suction cup in \cite{xu2022umpnet}), while our work learns an agent policy of a disembodied hand whose actions are continuous and close-loop in the simulated environment. 



==> 7Acknowledge.tex <==
\section{Acknowledgement}
We thank Gao Tang for his insightful discussions during the whole research process.

